A Disruptive Research Playbook for Studying Disruptive Innovations

As researchers, we are now witnessing a fundamental change in our technologically-enabled world due to the advent and diffusion of highly disruptive technologies such as generative AI, Augmented Reality (AR) and Virtual Reality (VR). In particular, software engineering has been profoundly affected by the transformative power of disruptive innovations for decades, with a significant impact of technical advancements on social dynamics due to its the socio-technical nature. In this paper, we reflect on the importance of formulating and addressing research in software engineering through a socio-technical lens, thus ensuring a holistic understanding of the complex phenomena in this field. We propose a research playbook with the goal of providing a guide to formulate compelling and socially relevant research questions and to identify the appropriate research strategies for empirical investigations, with an eye on the long-term implications of technologies or their use. We showcase how to apply the research playbook. Firstly, we show how it can be used retrospectively to reflect on a prior disruptive technology, Stack Overflow, and its impact on software development. Secondly, we show it can be used to question the impact of two current disruptive technologies: AI and AR/VR. Finally, we introduce a specialized GPT model to support the researcher in framing future investigations. We conclude by discussing the broader implications of adopting the playbook for both researchers and practitioners in software engineering and beyond.

==> notes.tex <==
% copying our notes here from main.tex

Notes from our discussion on June 8
\begin{itemize}
    \item McLhuan + McGrath we build upon since the beginning, in the intro. We might think about adding the revised table (slide 3 of \href{https://docs.google.com/presentation/d/1SJlVq0nIgD8YixxeVsAv6qcHZS8EMFO2mYSfegZ7bqA/edit?usp=sharing)}{Peggy's slides} as a motivating example 
    \item Nicole: add an example of how programming practice has changed (e.g., SO vs. Co-pilot, use of natural language)
    \item let's reflect on how to include consideration of other emerging technology (e.g. VR) as well as traditional machine learning into the big picture -> This could be shortly mentioned in the intro but then we can elaborate more in the discussion. The reason why we focus on LLM in this paper is because of it's disruptive: powerful + accessible (no specific knowledge required, low cost associated with their use). 
\end{itemize}


\textbf{Here is a link to our \href{https://docs.google.com/presentation/d/1d5IY0szvghyu3-psReFnns4Lb7Zi1Lqlh-8K0tmtfb0/edit?usp=sharing}{google doc} for convenience.}

Notes from our discussion Apr6:
\begin{itemize}
    \item Implications of AI - why we focus on this
    \item the ease at which the solutions can be built these days
    \item lots of economic forces - we have to stop and think - we can't just unleash this technology without considering the implications - what is missing is a framework to help guide this framework
    \item but just saying there are risks and not use it - is not realistic - it will be used - but just using it is not good either - so we need a way to use it but with reflection...  
    \item this framework has broader usage not just AI
    \item Aug 17 deadline for workshop proposals for IcSE 2024
    \item aim at a TOSEM fast track or maybe Communications of the ACM (if we have an in...)
    \item Research Problems instead of Research Questions... research directions or research lens or research focus... or research goals.... \textbf{Articulating Research Goals}....
    \item reminder for us - we need to make it clear how to make from theories to phenomena and research questions - we will have a diagram for this.... we can recommend novices to use chatgpt to generate these connections for people who are novice but again care must be taken but honestly Peggy prefer to have a guide for them to refer to :) we can check though how good chatgpt is... we know a lot...
    \item Let's change the first scenario from automatic program repair to program synthesis - similar to the co-pilot studies that have already been done -- come back to this in discussion how many papers that do this don't study enough phenomenon
    \item with program synthesis - the question of how the quality of the code will be effected over time (mcluhan) - we can look at papers on program synthesis and see which phenomena and research goals they consider...  likely not broad!
\end{itemize}
Notes from meeting Apr 13
\begin{itemize}
    \item the research questions as a compass
    \item are we focused on AI or LLMs (or automation!) - we have focused on automation in SE for 20 years but why propose this framework now and not 20 years ago - our line of reasoning can be of the highly disruptive nature of generative AI and with very few natural language prompts can generate text. Is it the interface (natural language) or underlying technology we are aiming at? We can think of LLMs more and more as an interface...  Is it about the more trust people are putting in it? With stackoverflow the signals of provenance and other opinions are visible by default, with chatGPT you can ask for the rational but you have to ask for it.  Do we want one of the examples to be more about ML? 
    \item reading for next week if we have these books or access to them :) O'Neil (Weapons of Math Destruction) and Mcluhan books/articles
    \item discussion about should we recommend using chatGPT for helping to find suitable theories for a question/phenomenon combination... we decided we will likely add this as a recommendation but with some guidance how to do so - to get the list of theories but then to consider which ones are more appropriate
    \item focus for next week is to talk about the scenarios (after a quick update on other sections)
\end{itemize}

Notes from meeting Apr 20
\begin{itemize}
    \item 
    %\url{https://tspace.library.utoronto.ca /bitstream/1807/87493/1/philosophies-01-00153-v2.pdf} 
    we should read this and recreate the table for software development
\item{ retrieval: LLM retried natural language descriptions -> pseudocode}
\item{ flip: all generated code is from generated code}
\end{itemize}

Notes from meeting Apr 27
\begin{itemize}
    \item will add the "table" to the paper - mering all three versions from peggy, nicole, takashi. . See %\url{https://docs.google.com/presentation/d/1rXD7GhB6wD_bjyaeNOcGEJPOZzwSwOMh/edit?usp=sharing&ouid=104615226548227850490&rtpof=true&sd=true}, \url{https://docs.google.com/presentation/d/1SJlVq0nIgD8YixxeVsAv6qcHZS8EMFO2mYSfegZ7bqA/edit?usp=sharing} and \url{https://docs.google.com/spreadsheets/d/19EyCO0wrP2F1cPGwcjJHYPpaD4484SK3aSd0VA3CkUU/edit?usp=sharing}.  [Action: Peggy/Nicole/Takashi]
    \item Peggy to work on research questions/framework section [Action: Peggy]
    \item Daniel to integrate thoughts from substantive/conceptual domain to the phenomena section (perhaps also mention unit of observation, and the Users, Artifacts, Environment dimension from the McLuhan section. Daniel to add "community" as a dimension. [Action: Daniel, Peggy can help/comment]
    \item Daniel to start working on theories section - more as a demonstration of what can be used - Dong mentioned he can help. [Action: Daniel/Dong]
    \item Nicole mentioned adding a table to provide an overview of the scenarios. [Action: Nicole]
    \item Japanese golden week next week - Dong and takashi will miss
    \item We will try to meet at ICSE and use Slack to coordinate. 
\end{itemize}

@article{CHATTERJEE2020110454,
title = {Finding help with programming errors: An exploratory study of novice software engineers’ focus in stack overflow posts},
journal = {Journal of Systems and Software},
volume = {159},
pages = {110454},
year = {2020},
issn = {0164-1212},
doi = {https://doi.org/10.1016/j.jss.2019.110454},
url = {https://www.sciencedirect.com/science/article/pii/S0164121219302286},
author = {Preetha Chatterjee and Minji Kong and Lori Pollock},
keywords = {Empirical study, Stack overflow, Mining software repositories, Software developer behavior},
}
